A retrospective analysis of Montana's 2020 congressional redistricting map

The 2020 decennial census data resulted in an increase from one to two congressional representatives in the state of Montana. The state underwent its redistricting process in 2021 in time for the November 2022 congressional elections, carving the state into two districts. This paper analyzes the redistricting process and compares the adopted congressional map to the space of all other possible maps. In particular, we look at the population deviation, compactness and political outcomes of these maps. We also consider how well two popular sampling techniques, that sample from the space of possible maps, approximate the true distributions of these measures.

==> mytable-old.tex <==
 \begin{table}[h!]
\caption{Lengths of borders between MT counties $< 50$ miles.}
\label{table:borderlengths}
\begin{tabular}{l|l|r|r|r}
\hline
\hline
C1 & C2 & miles & \% of C1 & \% of C2\\
\hline
\hline
Deer Lodge & Ravalli & 0.21 & 0.13 & 0.07\\
\hline
Custer & Garfield & 1.98 & 0.66 & 0.49\\
\hline
Meagher & Sweet Grass & 5.00 & 1.81 & 2.17\\
\hline
Rosebud & Yellowstone & 6.03 & 1.40 & 2.08\\
\hline
Golden Valley & Yellowstone & 13.84 & 7.64 & 4.77\\
\hline
Flathead & Missoula & 15.62 & 3.22 & 4.57\\
\hline
Deer Lodge & Jefferson & 16.11 & 9.68 & 7.45\\
\hline
Liberty & Pondera & 16.57 & 8.95 & 6.40\\
\hline
Gallatin & Jefferson & 19.48 & 5.78 & 9.00\\
\hline
Chouteau & Pondera & 20.04 & 5.96 & 7.74\\
\hline
Fallon & Prairie & 21.99 & 11.38 & 9.13\\
\hline
Carbon & Park & 22.80 & 8.59 & 7.91\\
\hline
Prairie & Wibaux & 24.67 & 10.24 & 14.48\\
\hline
Big Horn & Powder River & 26.39 & 6.45 & 11.22\\
\hline
Park & Stillwater & 26.56 & 9.22 & 10.56\\
\hline
Gallatin & Meagher & 26.61 & 7.89 & 9.62\\
\hline
Flathead & Powell & 30.66 & 6.31 & 10.15\\
\hline
Petroleum & Rosebud & 31.37 & 11.61 & 7.29\\
\hline
Fergus & Wheatland & 33.80 & 8.76 & 21.47\\
\hline
Fergus & Musselshell & 35.80 & 9.28 & 16.75\\
\hline
Chouteau & Judith Basin & 39.85 & 11.85 & 18.25\\
\hline
Chouteau & Teton & 39.97 & 11.89 & 15.35\\
\hline
Richland & Wibaux & 41.27 & 17.00 & 24.23\\
\hline
McCone & Richland & 41.80 & 14.99 & 17.22\\
\hline
Fergus & Golden Valley & 43.93 & 11.39 & 24.25\\
\hline
Garfield & Prairie & 44.30 & 10.99 & 18.40\\
\hline
Lewis and Clark & Meagher & 44.49 & 11.05 & 16.08\\
\hline
Deer Lodge & Powell & 45.75 & 27.48 & 15.14\\
\hline
Jefferson & Powell & 46.90 & 21.67 & 15.52\\
\hline
Golden Valley & Sweet Grass & 46.95 & 25.92 & 20.40\\
\hline
Missoula & Ravalli & 47.98 & 14.03 & 15.24\\
\hline
Carbon & Yellowstone & 48.94 & 18.44 & 16.85\\
\hline
Meagher & Park & 49.13 & 17.76 & 17.05\\
\hline
Flathead & Teton & 49.50 & 10.19 & 19.01\\
\hline
%Blaine & Chouteau & 55.30 & 17.34 & 16.45\\
%\hline
%Broadwater & Lewis and Clark & 58.62 & 28.06 & 14.56\\
%\hline
%Golden Valley & Stillwater & 59.11 & 32.63 & 23.50\\
%\hline
%Fallon & Wibaux & 59.26 & 30.67 & 34.80\\
%\hline
%Sweet Grass & Wheatland & 60.16 & 26.14 & 38.21\\
%\hline
%Petroleum & Phillips & 60.24 & 22.29 & 15.19\\
%\hline
%Judith Basin & Meagher & 60.25 & 27.59 & 21.78\\
%\hline
%Madison & Silver Bow & 60.60 & 20.90 & 37.93\\
%\hline
%Judith Basin & Wheatland & 61.63 & 28.23 & 39.15\\
%\hline
%Musselshell & Rosebud & 62.07 & 29.03 & 14.43\\
%\hline
%Flathead & Pondera & 63.08 & 12.98 & 24.37\\
%\hline
%Jefferson & Madison & 64.39 & 29.75 & 22.20\\
%\hline
%Daniels & Sheridan & 68.10 & 40.62 & 38.59\\
%\hline
%Meagher & Wheatland & 68.51 & 24.76 & 43.52\\
%\hline
%Beaverhead & Silver Bow & 68.69 & 13.14 & 43.00\\
%\hline
%Flathead & Sanders & 69.89 & 14.39 & 18.38\\
%\hline
%Chouteau & Liberty & 72.16 & 21.47 & 38.98\\
%\hline
%Glacier & Toole & 72.79 & 25.66 & 36.51\\
%\hline
%Jefferson & Lewis and Clark & 73.88 & 34.14 & 18.34\\
%\hline
%Flathead & Lewis and Clark & 73.99 & 15.23 & 18.37\\
%\hline
%Granite & Missoula & 74.04 & 33.69 & 21.64\\
%\hline
%Daniels & Roosevelt & 76.02 & 45.35 & 25.88\\
%\hline
%Musselshell & Petroleum & 76.22 & 35.65 & 28.20\\
%\hline
%Missoula & Sanders & 78.50 & 22.95 & 20.64\\
%\hline
%Beaverhead & Ravalli & 78.78 & 15.07 & 25.02\\
%\hline
%Roosevelt & Valley & 80.06 & 27.25 & 21.85\\
%\hline
%Stillwater & Yellowstone & 80.37 & 31.95 & 27.67\\
%\hline
%Fergus & Phillips & 81.77 & 21.19 & 20.62\\
%\hline
%Blaine & Fergus & 82.87 & 25.99 & 21.48\\
%\hline
%Big Horn & Treasure & 83.61 & 20.42 & 48.43\\
%\hline
%Custer & Fallon & 84.15 & 28.08 & 43.55\\
%\hline
%McCone & Roosevelt & 84.78 & 30.40 & 28.86\\
%\hline
%Beaverhead & Deer Lodge & 85.06 & 16.28 & 51.10\\
%\hline
%McCone & Prairie & 88.28 & 31.66 & 36.66\\
%\hline
%Garfield & Phillips & 89.05 & 22.08 & 22.45\\
%\hline
%Cascade & Teton & 89.45 & 28.50 & 34.36\\
%\hline
%Golden Valley & Wheatland & 90.76 & 50.10 & 57.65\\
%\hline
%Deer Lodge & Silver Bow & 92.05 & 55.30 & 57.63\\
%\hline
%Powder River & Rosebud & 93.33 & 39.66 & 21.69\\
%\hline
%Deer Lodge & Granite & 93.73 & 56.31 & 42.66\\
%\hline
%Daniels & Valley & 95.59 & 57.02 & 26.08\\
%\hline
%McCone & Valley & 97.54 & 34.98 & 26.62\\
%\hline
%Jefferson & Silver Bow & 98.15 & 45.36 & 61.44\\
%\hline
%Treasure & Yellowstone & 100.07 & 57.97 & 34.45\\
%\hline
%Dawson & McCone & 100.08 & 42.84 & 35.89\\
%\hline
%Broadwater & Gallatin & 106.59 & 51.03 & 31.61\\
%\hline
%Golden Valley & Musselshell & 107.74 & 59.47 & 50.40\\
%\hline
%Roosevelt & Sheridan & 108.93 & 37.08 & 61.74\\
%\hline
%Hill & Liberty & 108.94 & 43.02 & 58.85\\
%\hline
%Granite & Powell & 109.76 & 49.95 & 36.32\\
%\hline
%Dawson & Wibaux & 111.00 & 47.51 & 65.18\\
%\hline
%Broadwater & Jefferson & 113.89 & 54.52 & 52.63\\
%\hline
%Mineral & Sanders & 114.16 & 48.09 & 30.02\\
%\hline
%Carter & Powder River & 114.25 & 45.01 & 48.55\\
%\hline
%Carter & Fallon & 116.10 & 45.74 & 60.08\\
%\hline
%Cascade & Judith Basin & 116.12 & 36.99 & 53.18\\
%\hline
%Custer & Powder River & 116.66 & 38.92 & 49.57\\
%\hline
%Pondera & Toole & 117.48 & 45.39 & 58.92\\
%\hline
%Dawson & Prairie & 119.97 & 51.35 & 49.82\\
%\hline
%Missoula & Powell & 121.51 & 35.52 & 40.21\\
%\hline
%Liberty & Toole & 124.77 & 67.41 & 62.58\\
%\hline
%Cascade & Chouteau & 129.82 & 41.36 & 38.62\\
%\hline
%Glacier & Pondera & 131.66 & 46.42 & 50.87\\
%\hline
%Cascade & Lewis and Clark & 131.73 & 41.97 & 32.71\\
%\hline
%Blaine & Hill & 134.44 & 42.16 & 53.09\\
%\hline
%Dawson & Richland & 136.18 & 58.29 & 56.10\\
%\hline
%Broadwater & Meagher & 138.70 & 66.40 & 50.13\\
%\hline
%Mineral & Missoula & 139.64 & 58.82 & 40.82\\
%\hline
%Garfield & McCone & 145.19 & 36.00 & 52.07\\
%\hline
%Musselshell & Yellowstone & 145.72 & 68.17 & 50.17\\
%\hline
%Garfield & Valley & 148.12 & 36.73 & 40.42\\
%\hline
%Chouteau & Hill & 149.40 & 44.44 & 59.00\\
%\hline
%Lake & Missoula & 150.44 & 58.66 & 43.98\\
%\hline
%Big Horn & Carbon & 153.43 & 37.48 & 57.82\\
%\hline
%Lake & Sanders & 153.90 & 60.01 & 40.47\\
%\hline
%Carbon & Stillwater & 154.01 & 58.04 & 61.22\\
%\hline
%Custer & Rosebud & 156.67 & 52.27 & 36.42\\
%\hline
%Fergus & Judith Basin & 158.87 & 41.17 & 72.75\\
%\hline
%Cascade & Meagher & 160.67 & 51.19 & 58.07\\
%\hline
%Rosebud & Treasure & 161.59 & 37.56 & 93.60\\
%\hline
%Granite & Ravalli & 161.94 & 73.70 & 51.43\\
%\hline
%Park & Sweet Grass & 165.05 & 57.27 & 71.72\\
%\hline
%Chouteau & Fergus & 165.81 & 49.32 & 42.97\\
%\hline
%Pondera & Teton & 168.81 & 65.22 & 64.84\\
%\hline
%Fergus & Petroleum & 168.83 & 43.76 & 62.48\\
%\hline
%Lewis and Clark & Teton & 172.96 & 42.95 & 66.44\\
%\hline
%Garfield & Rosebud & 174.14 & 43.18 & 40.48\\
%\hline
%Big Horn & Rosebud & 175.24 & 42.80 & 40.73\\
%\hline
%Custer & Prairie & 182.43 & 60.86 & 75.75\\
%\hline
%Stillwater & Sweet Grass & 183.09 & 72.78 & 79.56\\
%\hline
%Richland & Roosevelt & 183.45 & 75.58 & 62.44\\
%\hline
%Big Horn & Yellowstone & 185.97 & 45.43 & 64.02\\
%\hline
%Gallatin & Park & 190.71 & 56.56 & 66.17\\
%\hline
%Gallatin & Madison & 191.45 & 56.77 & 66.02\\
%\hline
%Flathead & Glacier & 192.84 & 39.69 & 67.99\\
%\hline
%Lincoln & Sanders & 200.55 & 63.01 & 52.73\\
%\hline
%Garfield & Petroleum & 203.82 & 50.54 & 75.42\\
%\hline
%Flathead & Lincoln & 207.75 & 42.76 & 65.27\\
%\hline
%Flathead & Lake & 208.55 & 42.93 & 81.32\\
%\hline
%Phillips & Valley & 214.83 & 54.16 & 58.62\\
%\hline
%Beaverhead & Madison & 247.52 & 47.36 & 85.36\\
%\hline
%Lewis and Clark & Powell & 249.81 & 62.03 & 82.67\\
%\hline
%Blaine & Phillips & 251.57 & 78.89 & 63.43\\
\hline
\end{tabular}
\end{table}
